Polynomial-Time Power-Sum Decomposition of Polynomials

We give efficient algorithms for finding power-sum decomposition of an input polynomial $P(x)= \sum_{i\leq m} p_i(x)^d$ with component $p_i$s. The case of linear $p_i$s is equivalent to the well-studied tensor decomposition problem while the quadratic case occurs naturally in studying identifiability of non-spherical Gaussian mixtures from low-order moments. Unlike tensor decomposition, both the unique identifiability and algorithms for this problem are not well-understood. For the simplest setting of quadratic $p_i$s and $d=3$, prior work of Ge, Huang and Kakade yields an algorithm only when $m \leq \tilde{O}(\sqrt{n})$. On the other hand, the more general recent result of Garg, Kayal and Saha builds an algebraic approach to handle any $m=n^{O(1)}$ components but only when $d$ is large enough (while yielding no bounds for $d=3$ or even $d=100$) and only handles an inverse exponential noise. Our results obtain a substantial quantitative improvement on both the prior works above even in the base case of $d=3$ and quadratic $p_i$s. Specifically, our algorithm succeeds in decomposing a sum of $m \sim \tilde{O}(n)$ generic quadratic $p_i$s for $d=3$ and more generally the $d$th power-sum of $m \sim n^{2d/15}$ generic degree-$K$ polynomials for any $K \geq 2$. Our algorithm relies only on basic numerical linear algebraic primitives, is exact (i.e., obtain arbitrarily tiny error up to numerical precision), and handles an inverse polynomial noise when the $p_i$s have random Gaussian coefficients. Our main tool is a new method for extracting the linear span of $p_i$s by studying the linear subspace of low-order partial derivatives of the input $P$. For establishing polynomial stability of our algorithm in average-case, we prove inverse polynomial bounds on the smallest singular value of certain correlated random matrices with low-degree polynomial entries that arise in our analyses.

==> robust.tex <==
\subsection{Robust Intersection of Subspaces}

Above we have showed that the problem of finding the span of $\{A^t\}$ reduces to the problem of robustly finding the intersection of 2 subspaces. Recall that we are given two subspaces $V_1, V_2$ with the promise that they intersect in a $m$-dimensional subspace $W$, and we need to find $W$. Furthermore we want a robust algorithm to do so, in the sense that given \textit{perturbed} subspaces $\widetilde{V_1},\widetilde{V_2}$ find a subspace $\widetilde{W}$ that is close to $W$. 

We will assume that the subspaces are given to us by their projection matrix: $Proj(V) := VV^T$, where $V$ is a $n \times dim(V)$-matrix whose comlumns form an orthonormal basis for $V$. We will prove the following theorem in this section:

\begin{theorem}\label{thm:robust-int}
For all $n$ and $ m \leq k \leq n$, and for all $\delta,\epsilon \in (0,1)$ such that $\epsilon \ll \delta$ we have the following:
Let $V_1, V_2$ be two $k$-dimensional subspaces that are promised to intersect in a $m$-dimensional subspace $W$. Assume that $M = Proj(V_1)+Proj(V_2)$ is such that $\lambda_{m+1}(M) \leq 2 - \delta$.
Let $\widetilde{V_1},\widetilde{V_2}$ be perturbations of $V_1,V_2$ such that
$||Proj(\widetilde{V_i}) - Proj(V_i)||_F \leq \epsilon$. Then Algorithm 1 will recover a subspace $\widetilde{W}$ such that:
$$\Norm{Proj(W) - Proj(\widetilde{W})}_F \leq \epsilon',$$
where $\epsilon'$ is a function of $\epsilon,\delta,n$. 
\end{theorem}


Algorithm 1:
\begin{enumerate}
\item Consider the matrix $M = Proj(\widetilde{V_1}) + Proj(\widetilde{V_2})$.
\item Output the top $m$-dimensional eigenspace of $M$.
\end{enumerate}

\paragraph{Analysis:} First note that if $\epsilon = 0$ then every unit vector $w$ in the intersection of $V_1,V_2$ will satisfy $w^T M w = 2$. Furthermore, every vector $w \notin W$ will satisfy: $w^T M w < 2$. Hence the top eigenspace of $M$ will exactly be equal to $W$.

\mitali{rewrite the matrix perturbation theorem in our own words and cite correctly}

\paragraph{Robustness:} Let us now see why this algorithm is robust. This property follows from a modified version of Lemma G.5 of [HGK]. Roughly this lemma says that if we have a rank $k$ matrix $A$ and $W$ is the matrix of the top $k$ singular vectors, then for all perturbations $\widetilde{A}$ of $A$, the matrix $\widetilde{W}$ of the top-$k$ singular vectors of $\widetilde{A}$ will satisfy that $||Proj(W) - Proj(\widetilde{W})|| \leq \epsilon'$, which is a function of the minimum singular value of $A$ and the perturbation $\epsilon$.

\textbf{
Thus for our algorithm it suffices for $\lambda_{m+1}(M)$ to be bounded away from $\lambda_m(M) = 2$, since we are considering the top-$m$ dimensional eigenspace of $M$.} We will obtain $\widetilde{W}$ that is $\epsilon'$ close to $W$, where $\epsilon'$ depends on the eigenvalue gap $\delta$ and on the input perturbation $\epsilon$.


